AppIntent: Intuitive Automation Specification Framework for Mobile AppTesting

The proliferation of mobile apps and reduced time in mobile app releases mandates the need for faster and efficient testing of mobile apps, their GUI and functional capabilities. Though, there are wide variety of open source tools and frameworks that are developed to provide automated test infrastructure for testing mobile apps. Each of these automation tools supports different scripting languages for automating the app testing. These frameworks fundamentally lacks the ability to directly capture the intent of the users who intend to effectively test the mobile app and its cross-app functional capabilities and performance without worrying about the low-level scripting language associated with each tool. Hence, to address this limitation, we propose a high-level intent-based automation specification language and APIs that could effectively address following aspects: (i)capture the test automation steps to be captured as high-level intents using intuitive automation specification language, and (ii) provides framework support to effectively capture the users behavior patterns effectively for testing the apps. We develop, AppIntent a high level automation specification language-based framework that directly captures the test automation intents with in and across multiple apps using high-level and intuitive language without worrying about how to actually develop scripts for automation.

==> discussion_future.tex <==
%In this section, we describe about the limitations of our existing framework and potential for future enhancements to the tool and future research directions.

%This framework allows multiple tools to be integrated and the specification language that can be written abstracting out the underlying tools that are used for testing the tool. 

